Superpixel Transformers for Efficient Semantic Segmentation

Semantic segmentation, which aims to classify every pixel in an image, is a key task in machine perception, with many applications across robotics and autonomous driving. Due to the high dimensionality of this task, most existing approaches use local operations, such as convolutions, to generate per-pixel features. However, these methods are typically unable to effectively leverage global context information due to the high computational costs of operating on a dense image. In this work, we propose a solution to this issue by leveraging the idea of superpixels, an over-segmentation of the image, and applying them with a modern transformer framework. In particular, our model learns to decompose the pixel space into a spatially low dimensional superpixel space via a series of local cross-attentions. We then apply multi-head self-attention to the superpixels to enrich the superpixel features with global context and then directly produce a class prediction for each superpixel. Finally, we directly project the superpixel class predictions back into the pixel space using the associations between the superpixels and the image pixel features. Reasoning in the superpixel space allows our method to be substantially more computationally efficient compared to convolution-based decoder methods. Yet, our method achieves state-of-the-art performance in semantic segmentation due to the rich superpixel features generated by the global self-attention mechanism. Our experiments on Cityscapes and ADE20K demonstrate that our method matches the state of the art in terms of accuracy, while outperforming in terms of model parameters and latency.

==> tex/ade_qualitative.tex <==
\begin{figure*}[t!]
  \begin{center}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000010_sp_overlay.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000010_semantic_prediction.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000010_semantic_label.png}
  
  
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000048_sp_overlay.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000048_semantic_prediction.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000048_semantic_label.png}
  
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000063_sp_overlay.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000063_semantic_prediction.png}
  \includegraphics[width=0.25\linewidth]{images/ade_qualitative/000063_semantic_label.png}
  
  \end{center}
  \caption{Qualitative examples of our ConvNeXt-L backbone model on the ADE20K dataset. Left: Input image with superpixel boundaries overlaid. Middle: Semantic prediction. Right: Semantic ground truth. The superpixels are visualized by generating a hard assignment by taking the argmax of the soft assignment, and are best viewed zoomed in.}  
  \label{fig:ade_qualitative}   
\end{figure*}

==> tex/cityscapes_large_table.tex <==
\begin{table*} [t]
\centering
\begin{tabular}{l|c|ccc|c}
Method & Backbone & Params $\downarrow$ & FLOPs $\downarrow$ & FPS$ \uparrow$ & mIoU $\uparrow$ \\
\shline
MaskFormer~\cite{cheng2021per} & ResNet-101c & - & - & - & 81.4 \\
Mask2Former$^{\ddagger}$~\cite{cheng2022masked} & Swin-L~\cite{liu2021swin} & - & - & - & 83.3 \\
RegProxy$^*$~\cite{zhang2022semantic} & ViT-L/16~\cite{dosovitskiy2020image} & 307M & - & - & 81.4 \\
SegFormer~\cite{xie2021segformer} & MiT-B5~\cite{xie2021segformer} & \textbf{85M} & \textbf{1,448G} & 2.5 & 82.4 \\
SP-Transformer & ConvNeXt-L~\cite{liu2022convnet} & 202M & 1,557G & \textbf{3.6} & 83.1 \\
\hline

$k$MaX-DeepLab$^{\dagger}$~\cite{yu2022k} & ConvNeXt-L~\cite{liu2022convnet} & 232M & 1,673G & 3.1 & \textbf{83.5} \\
\end{tabular}
\caption{Cityscapes \textit{val} set results for large backbones. SP-Transformer achieves similar reductions in parameters, while achieving the lowest latency, and competitive mIoU performance. $^*$ RegProxy evaluates using a 768$^2$ sliding window. $^\dagger$\textit{k}MaX-DeepLab is trained for panoptic segmentation. $^\ddagger$Pretrained on ImageNet-22k.}
\label{tab:cityscapes_large}
\end{table*}
